Three-Loop Contributions to the Gluonic Massive Operator Matrix Elements at General Values of N

Recent results on the calculation of 3-loop massive operator matrix elements in case of one and two heavy quark masses are reported. They concern the $O(n_f T_F^2 C_{F,A})$ and $O(T_F^2 C_{F,A})$ gluonic corrections, two-mass quarkonic moments, and ladder- and Benz-topologies. We also discuss technical aspects of the calculations.

==> PaxHeaders.16975/paper.tex <==
20 atime=1357131652
20 ctime=1357131648

